Vertiport Navigation Requirements and Multisensor Architecture Considerations for Urban Air Mobility

Communication, Navigation and Surveillance (CNS) technologies are key enablers for future safe operation of drones in urban environments. However, the design of navigation technologies for these new applications is more challenging compared to e.g., civil aviation. On the one hand, the use cases and operations in urban environments are expected to have stringent requirements in terms of accuracy, integrity, continuity and availability. On the other hand, airborne sensors may not be based on high-quality equipment as in civil aviation and solutions need to rely on tighter multisensor solutions, whose safety is difficult to assess. In this work, we first provide some initial navigation requirements related to precision approach operations based on recently proposed vertiport designs. Then, we provide an overview of a possible multisensor navigation architecture solution able to support these types of operations and we comment on the challenges of each of the subsystems. Finally, initial proof of concept for some navigation sensor subsystems is presented based on flight trials performed during the German Aerospace Center (DLR) project HorizonUAM.

==> sections/5_campaign_old.tex <==
\hl{[CZ, YHL, WH, DG, MS, OG]}
%--------------------------------- TESTS, GENERAL ---------------------------------------
% Explain the experimental environment with figure: Cochstedt airport
\begin{figure*}
    \centering
    \includegraphics[trim={1cm 1.5cm 0.5cm 1cm},clip,width=\linewidth]{images/Cochstedt.png}
    \caption{Test set-up for navigation systems during HorizonUAM project in Cochstedt.}
    \label{fig:cochstedt}
\end{figure*}
\FloatBarrier
%
%TODO [yhlee->all] Picture of the platform (drone) with our sensor module??
%
%--------------------------------- U-GBAS TESTS ---------------------------------------
\subsection{U-GBAS}\label{subsec:ugbas_test}
\hl{[DG]}
% Some position and PL result from GBAS
%

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/GNSS_trajectory_04_07_23.png}
    \caption{Reference trajectory of short flights between Vertiport 1 and 2 in Figure~\ref{fig:cochstedt}.}
    \label{fig:UGBAS_ref_trajectory}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/UGBAS_live_PLs_PEs.png}
    \caption{Real-time protection levels based on close-by GNSS reference during take-off and landing operations.}
    \label{fig:UGBAS_PE_PLs_live}
\end{figure}
\FloatBarrier
%--------------------------------- BARO TESTS ---------------------------------------
\subsection{Ground-corrected barometer for vertiport operations}\label{subsec:baro_test}
\hl{[MS]} 
\paragraph{Test equipment}
During the flight trials, the airborne pressure measurements were performed by an Xsens MTi\textendash G\textendash 710 industrial grade navigation system. The ground measurements were read from the weather station and transmitted to the drone by a ground computer, specifically a Raspberry Pi 3 Model B. The data was transmitted over the WLAN provided by a router and locally extended with an additional antenna. The airborne and ground pressure measurements were processed by an airborne computer, an Intel® NUC 8 Pro Kit. Figure~\ref{fig:baro_results} gives a schematic representation of the system. 
%Details: serial connection VAISALA-Pi; sampling rate, resolution, and accuracy both of VAISALA and Xsens
% 
% location of weather station can be found in Fig 7.
%

%For the case of this specific implementation of the ground\textendash corrected approach, the fault tree of Subsection~\ref{subsec:baro_theory} would need to feature five top\textendash level branches corresponding to: the airborne barometer, the weather station and its power supply, the airborne computer, the ground computer, and the router and antenna assembly.
%Xsens  reports for the employed device a MTBF of 300000 hours, which correspond to a FR of 3.3 $\times 10^{-6}$ h$^{-1}$.
%Intel  provide for the NUC computer a MTBF of 50000 hours, corresponding to a FR of 2 $\times 10^{-5}$ h$^{-1}$. 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/Baro_system_hardware v10.png}
    \caption{Hardware side of the system for the computation of real-time ground-corrected pressure altitude during HorizonUAM tests.}
    \label{fig:baro_hardware}
\end{figure}

\paragraph{Calibration}
The employed airborne barometer is realistically of a notably lower grade if compared to barometers used in aviation or even to the one described in~\cite{Lerro2021} for UAM vehicles. For this reason, especially in this case, an adjustment of the airborne barometer measurements is needed. Biases could otherwise result in large altitude estimation errors. 

A comparison of a time series of pressure measurements of the adopted airborne barometer with the ones of the weather station showed an almost constant offset of approximately 193 Pa. A second comparison six weeks later showed an offset of 197 Pa. The employed airborne barometer and the weather station were factory\textendash calibrated several years ago and few months ago, respectively. 
%The weather station only produces air temperature and pressure measurements, while the barometer sensor is only one among several navigation sensors integrated in the Xsens Mti\textendash G\textendash 710. 
Based on this and on the specifications of these devices, it can be assumed the weather station to be more reliable. It can also be assumed that a constant bias of approximately 195 Pa 
%or a potentially slowly growing bias is
was present in the airborne barometer. This bias would translate to an absolute altitude offset of approximately 16 m, at ISA MSL conditions. We hence adjusted the airborne pressure measurements by removing this bias, before employing them for the barometric geodetic altitude computation. 

% In an operational scenario, we thus advocate the usage of regular inspection and calibration of reliable ground weather stations and airborne air pressure measuring systems. 
In an operational scenario, we recommend the usage of reliable and stable ground weather stations. We also advocate regular inspections and calibrations of airborne barometers, in case their stabilities and accuracies will be limited by industry requirements for reduced cost and mass.
 \FloatBarrier
\paragraph{Initial results}
The lower plot of Figure~\ref{fig:baro_results} presents some initial results of the barometric geodetic altitude computation based on the ground\textendash correction approach. The results represent several short flights over more than 30 minutes. 
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/baro_campaign.png}
    \caption{Pressure measurements (upper plot) and barometric geodetic altitude (lower plot) along HorizonUAM test flights.}
    \label{fig:baro_results}
\end{figure}
\FloatBarrier
The upper plot of Figure~\ref{fig:baro_results} shows the airborne and the vertiport pressure measurements. From this plot, it can be noticed that the employed method produces altitude measurements that quite well capture the true altitude profile. However, the barometric geodetic altitude shows a quite noisy behavior. This is due to the noise in the airborne pressure measurements, of a notably higher level than the one in the ground pressure measurements. The highest errors in the geodetic altitude computation are found in those transients during which the drone is flying very close to the ground. Despite these errors, the proposed approach shows first promising performances for vertical navigation in UAM applications.
%These errors are due to a confined increase in the air pressure around the airborne barometer. We suspect this increase to be the result of the interaction of the air flowing downwards from the spinning rotors with the close ground. Future analyses may potentially help deriving a model for the compensation of these effects.%, based on parameters such as altitude above ground, rotor velocity, vertical acceleration or others.
%Despite the aforementioned errors, the proposed approach shows first promising performances for reliable vertical navigation of UAVs in UAM applications.
%
%--------------------------------- VISION TESTS ---------------------------------------
\subsection{Camera-aided takeoff and landing}\label{subsec:camera_test}
\hl{[CZ, YHL, WH]}

% -------------
% Introduction
It is very challenging to achieve the navigation requirements only using GNSS during take-off and landing phases of UAM operations since vehicles fly close to the ground (vertiports). Thus, vision-based positioning was used to support those critical phases in the experimental environment. 

% -------------
% Setup of experiment of vision
For vision-aided positioning, two different AprilTag markers \cite{olson2011tags,wang2016iros,krogius2019iros} were generated using the family type "tag25h9" and pattern ID=11 and 21. A marker with pattern ID=11 was placed on the take-off site (Vertiport 1 in \figref{fig:cochstedt}), and the other one with ID=21 was placed on the landing site (Vertiport 2 in \figref{fig:cochstedt}). Both markers' size was equally set as $0.785\mathrm{m}\times0.785\mathrm{m}$.
Additionally, five smaller markers ($0.048\mathrm{m}\times0.048\mathrm{m}$) generated using the same family group (tag25h9) and patterns IDs=0$\sim$4 were placed on the bigger marker of the landing site (see \figref{subfig:multi_scale_marker_cut}). Using this multi-scale marker, the vehicle can still estimate its positions using the smaller marker detection results, although the bigger marker is no longer visible, as shown in \figref{subfig:apriltag_detection_smaller}. 


\begin{figure}[t]
    \centering
    \begin{subfigure}{\linewidth}
    \centering
        \includegraphics[width=.5\linewidth]{images/multi_scale_marker_cut.jpg}
        \caption{Multi-scale marker placed on the landing site. Bigger marker length=0.785m and smaller marker length=0.048m.}
        \label{subfig:multi_scale_marker_cut}
    \end{subfigure} \\
    %%
    \centering
    \begin{subfigure}[t]{.45\linewidth}
    \centering
        \includegraphics[width=\linewidth]{images/apriltag_detection_bigger.png}
        \caption{Bigger marker detection at higher altitude.}
        \label{subfig:apriltag_detection_bigger}
    \end{subfigure} ~~~
    %%%
    \begin{subfigure}[t]{.45\linewidth}
    \centering
        \includegraphics[width=\linewidth]{images/apriltag_detection_smaller.png}
        \caption{Smaller marker detection when the vehicle is close to the ground.}
        \label{subfig:apriltag_detection_smaller}
    \end{subfigure}
    \caption{Multi-scale marker design.}
    \label{fig:marker_design}
\end{figure}


% -------------
\paragraph{Error analysis of camera intrinsic parameter estimation} 
% As stated in Section \ref{subsec:limitations}, a critical limitation of vision-based navigation is that there is no reliable way to quantify and monitor the integrity of visual navigation. In order to monitor the integrity, we need to first model the errors in each step. Camera calibration is an essential step in almost all vision-based localization applications that require high accuracy. 
% In navigation tasks, the error in camera intrinsic parameters is propagated into the pose estimates. As a result, the quality of the calibration directly affects the positioning or localization performance. 
% Calibration errors are caused by the inevitable mismatch between the applied camera model and the reality as well as the measurement noise in the calibration process. If the calibration errors are overly optimistically considered or even ignored in vision-based navigation, it can lead to integrity risks. Therefore, it is important to model the calibration error appropriately in order to improve the performance of camera pose/motion estimation in terms of accuracy and integrity.

% In real-world scenarios, the actual (true) intrinsic parameters of a camera are not known. Typically, the intrinsic parameters are calibrated in a controlled environment, and assumed to remain constant after calibration. Despite the well-controlled environment, it’s not possible to completely eliminate all errors during the calibration process. In the experiment, we discovered that the intrinsic parameters have a significant impact on the camera position estimation. As shown in Figure \ref{fig:uncertaity-ellipse}, we conduct a simulation to see how the calibration error influence the camera position estimation uncertainty. The green ellipses represent the uncertainty distribution of the camera position with considering the impact of calibration uncertainty, while the red ellipses depict the uncertainty without considering the impact of calibration uncertainty. Figure \ref{fig:uncertaity-ellipse} clearly indicates that the calibration uncertainty greatly contributes to the camera position uncertainty.

% Marker-based positioning is with respect to the local frame with respect to the marker frame (origin at the marker center), so we geo-referenced the corners of the markers, so that we can convert the trajectory with respect to the local marker frame to the ECEF later to be able to enter the solutions to the air traffic management, and further possibility to fuse with GNSS solutions.
% %TODO add detail specs of the geo-referencing receivers

%TODO [yhlee->all] Maybe we could just simply say the errors of the intrinsic params have a big impact (?)
% \figref{fig:uncertainty-ellipse} shows the confidence error ellipses of the camera position estimates. The green ellipses represent the uncertainty distribution of the camera position with considering the impact of calibration uncertainty, while the red ellipses depict the uncertainty without considering the impact of calibration uncertainty. As shown in this figure, if we do not consider that camera calibration errors, we obtain the smaller error ellipse (as the red ellipses), although the actual error ellipses should be bigger as shown in green, since the calibration errors acutually exist. 

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{images/ellipse_close.png}
%          \caption{Camera is close to the marker points (3m).}
%          \label{fig:y equals x}
%      \end{subfigure}

%      \begin{subfigure}[b]{\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{images/ellipse_far.png}
%          \caption{Camera is far away from the marker points (7m).}
%          \label{fig:three sin x}
%      \end{subfigure}
%         \caption{Confidence ellipses of camera position uncertainty (green ellipse: with calibration uncertainty, red ellipse: without calibration uncertainty).}
%         \label{fig:uncertainty-ellipse}
% \end{figure}

% We used a monocular camera (FLIR Blackfly GigE Camera) to observe the markers. 
Before the flight experiments, the camera intrinsic parameters, such as focal length and the position of the optical center point, were estimated (camera calibration process). Then, the errors of the estimates were first analyzed since they have a significant impact on the camera position estimation \cite{hao2023camera}. 
First, multiple ArUco markers \cite{aruco} were installed on the ground as shown in \figref{fig:cam-calibration}. One of corner points was defined as the origin of the reference frame, and the true 3D locations of the other markers' corner points were computed with respect to the reference frame by measuring the distances between the markers. Then, sample images were obtained using the camera, and corner points were detected in the images.
The 3D coordinates of each corner points can be reconstructed with respect to the reference frame, using the camera intrinsic parameters (estimated during the calibration process) and the detected corner points. Finally, the differences between the reconstructed coordinates and the true 3D locations can be computed, and then back-propagated to the intrinsic parameters. With the estimated uncertainty in the calibrated intrinsic parameters using the above calibration test process, the quality of the camera calibration can be evaluated. If the uncertainty exceeds the required accuracy, the camera shall be re-calibrated. Otherwise, the calibration results are accepted, and the uncertainty in the intrinsic parameters are propagated to the position estimates and included in the protection level calculation. It has been shown through simulations that such calibration residual error can have significant impacts on the positioning uncertainty. The more detail processes and results can be found in our previous study \cite{hao2023camera}. 
%TODO [yhlee->cz] more explanation needed (we need to conclude the analysis here): analysis of the intrinsic parameter errors maybe with the following figures?
%TODO [yhlee->cz] 1) add a Fig related to the 3D location errors?
%TODO [yhlee->cz] 2) add a Fig related to the intrinsic parameter?
% CZ->YHL For detailed results I will just explain a bit and cross-refer to the Wenhan's PLANS paper instead of reincluding the images.

\begin{figure}[t]
    \centering
    \includegraphics[width=.85\linewidth]{images/markers05.jpg}
    \caption{Setup for the camera calibration error analysis (7 AruCo markers; marker IDs: $21\sim27$; marker size: $5\times5$ bits).}
    \label{fig:cam-calibration}
\end{figure}

% -------------
\paragraph{Analysis of positioning accuracy}
In the experiments, the vehicle took off at the Vertiport 1, flew the planned trajectory, and then landed on the Vertiport 2. The ground truth trajectory (gray in \figref{fig:trajectory_apriltag_vs_gnss}) were obtained using the differential correction method with GNSS as well as GBAS signals, and the decimeter level accuracy is expected. 
During the take-off and landing phases, the 3D positions of the vehicle were estimated using the markers placed on each vertiport. The position estimates are shown with colorbar in \figref{fig:trajectory_apriltag_vs_gnss}. 
As can be seen in the figure, the vehicle's trajectory was accurately estimated using the marker-based method during the both phases, following the ground truth trajectory within meter level differences. Moreover, we were able to estimate the vehicle's positions using the smaller markers when the vehicle was close to the ground (altitude lower than 1m).

%TODO [yhlee] only remain this figure
\begin{figure}[t]
    \centering
    \includegraphics[width=.98\linewidth]{images/trajectory_apriltag_vs_gnss_3d.png}
    \caption{Vision-based trajectory estimates during take-off (Vertiport 1) and landing (Vertiport 2) phases (colorbar). Ground truth trajectory is depicted with gray.}
    \label{fig:trajectory_apriltag_vs_gnss}
\end{figure}





==> sections/7_discussion.tex <==
\hl{[TBD whether we need this section, ...]}

% Discussions should be brief and focused. In some disciplines use of Discussion or `Conclusion' is interchangeable. It is not mandatory to use both. Some journals prefer a section `Results and Discussion' followed by a section `Conclusion'. Please refer to Journal-level guidance for any specific requirements. 
